Evading Deep Learning-Based Malware Detectors via Obfuscation: A Deep Reinforcement Learning Approach

Adversarial Malware Generation (AMG), the generation of adversarial malware variants to strengthen Deep Learning (DL)-based malware detectors has emerged as a crucial tool in the development of proactive cyberdefense. However, the majority of extant works offer subtle perturbations or additions to executable files and do not explore full-file obfuscation. In this study, we show that an open-source encryption tool coupled with a Reinforcement Learning (RL) framework can successfully obfuscate malware to evade state-of-the-art malware detection engines and outperform techniques that use advanced modification methods. Our results show that the proposed method improves the evasion rate from 27%-49% compared to widely-used state-of-the-art reinforcement learning-based methods.

==> table/exp_sum2.tex <==
\def\cellPadding{10pt}

\begin{table}[h!]
\caption{Summary of Experiments}
\label{expOverview}

\begin{tabular}{|m{0.75cm}<{\centering}
                |m{0.75cm}<{\centering}
                |m{2.3cm}<{\centering}
                |m{1.2cm}<{\centering}|}

    \hline

    \multicolumn{2}{|c|}{\textbf{Experiment}} & \multicolumn{2}{c|}{\textbf{Description}}\\ 

    \hline
    \vspace{\cellPadding} \vspace{\cellPadding} \multirow{2}{*}{Exp \#1} & \vspace{\cellPadding} \#1-1\ \vspace{\cellPadding} & \multirow{2}{*}{\parbox{2cm} {\centering Evaluation of OBFU-mal and several advanced AMG benchmark methods against:}} & MalConv\\

    \cline{2-2}\cline{4-4}
    
     & \vspace{\cellPadding} \#1-2 \vspace{\cellPadding} & & \hspace{-10pt}LightGBM/EMBER\\
     
    \hline
    
    \multicolumn{2}{|c|}{Exp \#2} & \multicolumn{2}{c|}{Qualitative analysis of evasive action sequences} \\ 
    
    \hline
    
    \multicolumn{2}{|c|}{Exp \#3} & \multicolumn{2}{c|}{Ablation analysis of OBFU-mal} \\ 
    
    \hline
    
\end{tabular}
\end{table}


% \begin{tabular}{|c|c|p{3.3cm}|c|}

% \hline

% \multicolumn{2}{|c|}{\textbf{Experiment}} & \multicolumn{2}{c|}{\textbf{Description}}          \\ 

% \hline

% & \#1-1 & & MalConv

% \hline

% \multirow{2}{*}[2ex]{Exp \#1} & \#1-2 & \multirow{2}{3.3cm}{Evaluation of OBFU-mal and several advanced AMG benchmark methods against:} & MalConv

% \multicolumn{2}{|c|}{Exp \#2} & \multicolumn{2}{c|}{Qualitative analysis of evasive action sequences} \\ 
% \hline

% \multicolumn{2}{|c|}{Exp \#3} & \multicolumn{2}{c|}{Ablation analysis of OBFU-mal} \\ 
% \hline
% \end{tabular}

==> table/exp_sum3.tex <==
\begin{table}[h]
\centering
\renewcommand{\arraystretch}{1.5} % Adjust the value as needed
\caption{Summary of Experiments}
\label{expOverview}
\begin{tabular}{|c|c|m{3.3cm}|c|}
\hline
\multicolumn{2}{|c|}{\textbf{Experiment}} & \multicolumn{2}{c|}{\textbf{Description}} \\
\hline
\multirow{2}{*}{\centering Exp \#1} & \#1-1 & \multirow{2}{3.3cm}{\centering Evaluation of OBFU-mal and several advanced AMG benchmark methods against:} & MalConv \\
\cline{2-2} \cline{4-4}
& \#1-2 & & LightGBM/EMBER \\
\hline
\multicolumn{2}{|c|}{Exp \#2} & \multicolumn{2}{c|}{Qualitative analysis of evasive action sequences} \\
\hline
\multicolumn{2}{|c|}{Exp \#3} & \multicolumn{2}{c|}{Ablation analysis of OBFU-mal} \\
\hline
\end{tabular}
\vspace{-5mm}
\end{table}

==> table/old_t7_malconv_obfu.tex <==
\begin{table*}[!ht]
\centering
\renewcommand{\arraystretch}{1.2}
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{-10mm}
\caption{Evasion Rate Result of OBFU-mal Samples Against MalConv Benchmark AMG Tactics}
\label{malconvEvasion}
\begin{tabular}{|c|c|c|c|c|c|c|c|}

\hline

\textbf{Tactic}                    & \textbf{Adware}  & \textbf{Botnet}  & \textbf{Ransomware} & \textbf{Rootkit} & \textbf{Spyware} & \textbf{Virus}   & \textbf{Average} \\ \hline
ACER      & 17.57\%          & 37.07\%          & 25.33\%             & 29.41\%          & 56.09\%          & 44.76\%          & 35.04\%          \\ \hline
Random Append & 2.06\%           & 2.47\%           & 3.78\%              & 4.73\%           & 2.50\%           & 1.88\%           & 2.79\%           \\ \hline
BFA   & 0.87\%           & 1.14\%           & 0.11\%              & 3.77\%           & 1.88\%           & 2.43\%           & 1.27\%           \\ \hline
Enhanced-BFA  & 15.51\%          & 21.86\%          & 14.44\%             & 3.77\%           & 11.50\%          & 12.29\%          & 15.86\%          \\ \hline
GAMMA      & 1.77\%           & 3.51\%           & 1.79\%              & 0\%              & 1.86\%           & 1.35\%           & 1.70\%           \\ \hline
MalGPT       & 25.89\%          & 25.86\%          & 20.33\%             & 24.53\%          & 22.97\%          & 28.38\%          & 24.51\%          \\ \hline
MAB-malware   & 64.18\%          & 52.93\%          & 48.38\%             & 45.23\%          & 50.99\%          & 55.96\%          & 50.70\%          \\ \hline
\textbf{OBFU-mal (Ours)}           & \textbf{66.62\%} & \textbf{69.58\%} & \textbf{56.89\%}    & \textbf{57.80\%} & \textbf{66.04\%} & \textbf{75.42\%} & \textbf{65.15\%} \\ \hline

\end{tabular}
% \vspace{-5mm}
\end{table*}

==> table/t10_lgbm_obfu_filesize.tex <==
\begin{table*}[!h]
\centering
\renewcommand{\arraystretch}{1.2}
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{-10mm}
\caption{File Size Increase in Malware Modified by OBFU-mal with Respect to LightGBM}
\label{lgbmFileSize}
\begin{tabular}{|c|c|c|c|c|}

\hline
\textbf{Type} & \textbf{\# of Samples} & \textbf{Avg Base File Size (kB)} & \textbf{Avg Mod File Size (kB)} & \textbf{Avg Increase in File Size} \\ \hline
Botnet        & 443                    & 241.00                           & 1933.67                         & 1179.47\%                          \\ \hline
Ransomware    & 565                    & 571.55                           & 3257.61                         & 545.07\%                           \\ \hline
Rootkit       & 570                    & 659.89                           & 4608.83                         & 747.45\%                           \\ \hline
Spyware       & 432                    & 639.97                           & 3980.83                         & 932.21\%                           \\ \hline
Virus         & 382                    & 33.86                            & 2587.06                         & 947.52\%                           \\ \hline

\end{tabular}
% \vspace{-5mm}
\end{table*}

==> table/t5_detectors.tex <==
\begin{table*}[!ht]
\centering
\renewcommand{\arraystretch}{1.2}
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{-10mm}

\caption{Malware Detectors}
\label{malwareDetectors}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Malware Detector} & \textbf{Owner} & \textbf{Type} & \textbf{Method} & \textbf{Input Data Type} & \textbf{References} \\
\hline
MalConv & Laboratory for Physical Sciences & DL-Based & CNN & First 2M input bytes & Raff et al. \cite{raff2018a} \\
\hline
LightGBM & Microsoft & Signature-Based & GBDT & 2,381 features from binary files & Anderson et al. \cite{anderson2018a} \\
\hline
\end{tabular}
% \vspace{-5mm}
\end{table*}

==> table/t8_malconv_obfu_filesize.tex <==
\begin{table*}[!ht]
\centering
\renewcommand{\arraystretch}{1.2}
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{-10mm}
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{-10mm}
\caption{File Size Increase in Malware Modified by OBFU-mal with Respect to MalConv}
\label{malconvObfuFileSizeIncrease}
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Type} & \textbf{\# of Samples} & \textbf{Avg Base File Size (kB)} & \textbf{Avg Mod File Size (kB)} & \textbf{Avg Increase in File Size} \\ \hline
Adware        & 1,947                  & 620.22                           & 2172.25                         & 297.64\%                           \\ \hline
Botnet        & 526                    & 241.00                           & 1460.42                         & 727.08\%                           \\ \hline
Ransomware    & 900                    & 571.55                           & 1792.78                         & 285.64\%                           \\ \hline
Rootkit       & 731                    & 659.98                           & 2847.4                          & 407.06\%                           \\ \hline
Spyware       & 640                    & 639.97                           & 2113.37                         & 455.53\%                           \\ \hline
Virus         & 659                    & 324.40                           & 1338.58                         & 744.22\%                           \\ \hline
\end{tabular}
% \vspace{-5mm}
\end{table*}

==> table/t9_lgbm_obfu.tex <==
\begin{table*}[!h]
\centering
\renewcommand{\arraystretch}{1.2}
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{-10mm}
\caption{OBFU-mal Evasion Rates Against LGBM/EMBER Benchmarks and Related Works}
\label{lgbmEvasion}
\begin{tabular}{|c|c|c|c|c|c|c|}

\hline
\textbf{Tactic} & \textbf{Botnet} & \textbf{Ransomware} & \textbf{Rootkit} & \textbf{Spyware} & \textbf{Virus} & \textbf{Average} \\ \hline
DDQN & 23.00\% & 44.33\% & 39.12\% & 19.80\% & 27.77\% & 28.44\% \\ \hline
ACER & 30.99\% & 60.11\% & 27.51\% & 26.87\% & 62.82\% & 37.18\% \\ \hline
Enhanced-BFA & 3.02\% & 4.44\% & 4.73\% & 5.34\% & 6.16\% & 3.90\% \\ \hline
AMG-VAC  & 48.29\% & 65.22 \% & 61.15\% & 29.53\% & \textbf{82.40\%} & 51.67\% \\ \hline
MAB-malware & 4.21\% & 11.25\% & 4.89\% & 10.98\% & 24.13\% & 11.09\% \\ \hline
\textbf{OBFU-mal (Ours)} & \textbf{67.32\%} & \textbf{92.44\%} & \textbf{81.48\%} & \textbf{88.07\%} & 63.46\% & \textbf{79.2\%} \\ \hline

\end{tabular}
% \vspace{-5mm}
\end{table*}
